ToolQA: A Dataset for LLM Question Answering with External Tools

Large Language Models (LLMs) have demonstrated impressive performance in various NLP tasks, but they still suffer from challenges such as hallucination and weak numerical reasoning. To overcome these challenges, external tools can be used to enhance LLMs' question-answering abilities. However, current evaluation methods do not distinguish between questions that can be answered using LLMs' internal knowledge and those that require external information through tool use. To address this issue, we introduce a new dataset called ToolQA, which is designed to faithfully evaluate LLMs' ability to use external tools for question answering. Our development of ToolQA involved a scalable, automated process for dataset curation, along with 13 specialized tools designed for interaction with external knowledge in order to answer questions. Importantly, we strive to minimize the overlap between our benchmark data and LLMs' pre-training data, enabling a more precise evaluation of LLMs' tool-use reasoning abilities. We conducted an in-depth diagnosis of existing tool-use LLMs to highlight their strengths, weaknesses, and potential improvements. Our findings set a new benchmark for evaluating LLMs and suggest new directions for future advancements. Our data and code are freely available to the broader scientific community on GitHub.

==> sections/plan.tex <==
% \input{sections/tab-related}
\section{Introduction}




The tools include:
\begin{itemize}
    \item Text: \cancel{Retriever}
    \item Table: SQL/pandas (filter, table grounding)
    \item Code:
    \item Math: \cancel{Calculator}
    \item Graph Tools
\end{itemize}

The prompts include:
\begin{itemize}
    \item Toolformer: \cancel{overall}, tool description
    \item ReAct: Zero-shot, Few-shot
    \item Chameleon: add ordering information in tool description.
\end{itemize}

\section{Difference with API-Bank}
The difference between our work and API-Bank can be summarized as follows:
\begin{enumerate}
    \item API-Bank only contains 8 toolchains for complicated tasks;
    \item API-Bank's tasks are all related to the personal assistant, which is more likely to be understood/included in training data;
    \item The solutions are fixed for each task and they offer the entire solution sequence.
\end{enumerate}

\section{Cases}
\subsection{Questions}
The questions seem to need further polish:
1. The performance on GSM8K seems to improve a lot over time. I select all the questions that the previous chatgpt cannot answer correctly. But now, over these questions, ChatGPT can achieve 22$\%$ accuracy.


\begin{table}[h]
\centering 
\renewcommand\arraystretch{0.88}
\fontsize{8}{10}\selectfont \setlength{\tabcolsep}{0.3em}
\begin{tabular}{@{}p{0.3\linewidth}|p{0.15\linewidth}|p{0.5\linewidth}@{}}
\toprule
Question & Ground-Truth & Model Prediction \\ \midrule
(Yelp-Easy) What is the address of Ebenezer Maxwell Mansion? & 200 W Tulpehocken St & 200 W Tulpehocken St, Philadelphia, PA 19144, United States. \\\midrule
(SciREX-Easy) What is the corresponding Percentage$\_$correct score of the ResNet method on CIFAR-10 dataset for Image$\_$Classification task? & 93.57 & The corresponding Percentage$\_$correct score of the ResNet method on CIFAR-10 dataset for Image$\_$Classification task is 95.92$\%$. \\\midrule
(Yelp-Easy) What are the categories that Coleman Worldwide Moving belong to? & Home Services, Movers & Coleman Worldwide Moving belongs to the category of moving and storage companies. \\\midrule
(Yelp-Easy) What is the postal code of Redington Long Pier in Redington Shores, FL? & 33708 & The postal code of Redington Shores, FL is 33708. \\ \bottomrule
\end{tabular}
\caption{The correct questions of ChatGPT-based answers correctly.}
\end{table}


\subsection{Judges}
The ChatGPT-based judgers can make mistakes: 

\begin{table}[h]
\centering 
\renewcommand\arraystretch{0.88}
\fontsize{8}{10}\selectfont \setlength{\tabcolsep}{0.3em}
\begin{tabular}{@{}p{0.3\linewidth}|p{0.15\linewidth}|p{0.5\linewidth}@{}}
\toprule
Question & Ground-Truth & Model Prediction \\ \midrule
(Flight-Easy) Was the flight AA1411 from PHL to DFW cancelled on 2022-01-20? & No & I do not have access to real-time flight information. Please check with the airline or visit the flight status website for accurate and up-to-date information. \\\midrule
(SciREX-Easy) What is the corresponding Percentage$\_$correct score of the ResNet method on CIFAR-10 dataset for Image$\_$Classification task? & 93.57 & The corresponding Percentage$\_$correct score of the ResNet method on CIFAR-10 dataset for Image$\_$Classification task is 95.92$\%$. \\\midrule
(Yelp-Easy) What state is Swarovski located in? & AB & Swarovski is not a state, it is an Austrian company. \\\midrule
(Agenda-Hard) Who is unavailble between 5:00 PM and 7:00 PM on 2022/09/31 in the agenda table?  & 6 & There is no 2022/09/31 as September only has 30 days. \\ \midrule
(Agenda-Hard) When should I schedule a meeting with Georgia from 9:00 AM to 6:00 PM on 2022/05/29 in the agenda table? & 9:00 AM-10:00 AM, 1:00 PM-6:00 PM & The meeting can be scheduled at any time between 9:00 AM to 6:00 PM on May 29th, 2022 based on individual or team availability. \\ \midrule
(Coffee-Hard) What was the highest coffee price from 2016-07-21 to 2017-06-06? & 176.0 USD & The highest coffee price during that time period was $\$$1.76 per pound.\\\bottomrule
\end{tabular}
\caption{The mistakes of ChatGPT-based judgers.}
\end{table}


\section{Research Plan}

\subsection{TODO List}
\begin{enumerate}
    \item Finalize the data. May need all of you to go through the question templates in the appendix and give some suggestions.
    \item Decide if we still need additional data in the benchmark.
    \item Decide what baselines to run first.
\end{enumerate}

\subsection{Progress}

\begin{itemize}
    \item 2023-05-10, add the synthetic agenda data and wrapup all the question-answer pairs. Start testing on ChatGPT.
    \item 2023-05-01, wrap up the supportive materials and summarize the research plans.
    \item 2023-04-28, wrap up an initial version of question-answer pairs.
\end{itemize}

\subsection{Main Results}
\subsubsection{Easy}
\begin{table}[h]
\centering 
\renewcommand\arraystretch{0.88}
\fontsize{8}{10}\selectfont \setlength{\tabcolsep}{0.3em}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
                & Flight & Coffee & Agenda & Yelp & Airbnb & DBLP & SciREX & GSM8K \\ \midrule
ChatGPT         &  2  &   0     &  0      &  15    &  0      & 0     &   2     &  22$\to$26     \\
Zero-Shot ReAct &        &        &        &      &        &      &        &       \\
Few-Shot ReAct  &        &        &        &      &        &      &        &       \\
ToolFormer      &        &        &        &      &        &      &        &       \\
Chameleon       &        &        &        &      &        &      &        &       \\
HuggingGPT      &        &        &        &      &        &      &        &       \\ \bottomrule
\end{tabular}
\end{table}


\subsubsection{Hard}
\begin{table}[h]
\centering 
\renewcommand\arraystretch{0.88}
\fontsize{8}{10}\selectfont \setlength{\tabcolsep}{0.3em}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
                & Flight & Coffee & Agenda & Yelp & Airbnb & DBLP & SciREX \\ \midrule
ChatGPT         &  3$\to$2      &   4.62$\to$2.31     &   4$\to$1     &  2$\to$0    &   2     &  6$\to$4    &    33    \\
Zero-Shot ReAct &        &        &        &      &        &      &        \\
Few-Shot ReAct  &        &        &        &      &        &      &      \\
ToolFormer      &        &        &        &      &        &      &       \\
Chameleon       &        &        &        &      &        &      &         \\
HuggingGPT      &        &        &        &      &        &      &        \\ \bottomrule
\end{tabular}
\end{table}

\subsection{Expert Comparison}
\subsubsection{Easy}
\begin{table}[h]
\centering 
\renewcommand\arraystretch{0.88}
\fontsize{8}{10}\selectfont \setlength{\tabcolsep}{0.3em}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
                & Flight & Coffee & Agenda & Yelp & Airbnb & DBLP & SciREX & GSM8K \\ \midrule
ToolFormer         &        &        &        &      &        &      &        &       \\
PAL &        &        &        &      &        &      &        &       \\
Graph-Toolformer  &        &        &        &      &        &      &        &       \\
Self-Debugging     &        &        &        &      &        &      &        &       \\
Program-of-Thoughts       &        &        &        &      &        &      &        &       \\\bottomrule
\end{tabular}
\end{table}


\subsubsection{Hard}
\begin{table}[h]
\centering 
\renewcommand\arraystretch{0.88}
\fontsize{8}{10}\selectfont \setlength{\tabcolsep}{0.3em}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
                & Flight & Coffee & Agenda & Yelp & Airbnb & DBLP & SciREX & GSM8K \\ \midrule
ToolFormer         &        &        &        &      &        &      &        &       \\
PAL &        &        &        &      &        &      &        &       \\
Graph-Toolformer  &        &        &        &      &        &      &        &       \\
Self-Debugging     &        &        &        &      &        &      &        &       \\
Program-of-Thoughts       &        &        &        &      &        &      &        &       \\\bottomrule
\end{tabular}
\end{table}

\subsection{Dataset Construction}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering 
\renewcommand\arraystretch{0.88}
\fontsize{8}{10}\selectfont \setlength{\tabcolsep}{0.2em}
\begin{tabular}{@{}cccccccc@{}}
\toprule
\multirow{2}{*}{Domain}   & \multirow{2}{*}{Topic} & \multicolumn{2}{c}{Corpus} & \multicolumn{2}{c}{Easy}    & \multicolumn{2}{c}{Hard}    \\ \cmidrule(l){3-8} 
                          &                        & Format      & Size         & \# Templates & \# Questions & \# Templates & \# Questions \\ \midrule
\multirow{3}{*}{Temporal} & Flight                 & csv         & 4078318      & 10           & 100          & 10           & 100          \\
                          & Coffee                 & csv         & 5746         & 8            & 100          & 13           & 130          \\
                          & Agenda           & text        &  10000     &  5      &  100            &  5       & 100      \\
\multirow{2}{*}{Spatial}  & Yelp                   & json        & 150346       & 11           & 100          & 10           & 100          \\
                          & Airbnb                 & json        & 102599       & 10           & 100          & 10           & 100          \\
Social                    & DBLP                   & graph       & 553320       & 10           & 100          & 10           & 100          \\
Expert          & SciREX                 & text        & 438          & 1            & 100          & 4            & 100          \\
Math & GSM8K & - & - & - & 100 & - & - \\\midrule
\textbf{Sum} & - & - & - & \textbf{55} & \textbf{800} & \textbf{62} & \textbf{730}\\\bottomrule
\end{tabular}
\end{table}

\subsubsection{Data Resources}

\begin{itemize}
    \item \textbf{Flight Status (2022-2023)}, link: \url{https://www.kaggle.com/datasets/robikscube/flight-delay-dataset-20182022?select=Combined_Flights_2022.csv}. This dataset contains all flight information including cancellation and delays by airline for dates between 2022 and 2023.
    \item \textbf{Daily Coffee Price (2000-2022)}, link: \url{https://www.kaggle.com/datasets/psycon/daily-coffee-price}. This dataset contains daily price of coffee price.
    \item \textbf{Yelp Business Data}, link: \url{https://www.kaggle.com/datasets/yelp-dataset/yelp-dataset?select=yelp_academic_dataset_business.json}. This dataset is subset of Yelp's business data. In the most recent dataset, you'll find information about businesses across 8 metropolitan areas in the USA and Canada.
    \item \textbf{Airbnb Open Data}, link: \url{https://www.kaggle.com/datasets/arianazmoudeh/airbnbopendata}. This dataset is a subset of Airbnb activities in New York. Following actions are included in the dataset: Listings, including full descriptions and average review score Reviews, including unique id for each reviewer and detailed comments Calendar, including listing id and the price and availability for that day.
    \item \textbf{DBLP Citation Network (V14)}, link: \url{https://www.aminer.org/citation}. We construct the graph based on the records in this dataset after 2020. The author-author and paper-paper relations are formulated as two separated graphs.
    \item \textbf{GSM8k}, link: \url{https://github.com/openai/grade-school-math}. GSM8K is a dataset of 8.5K high quality linguistically diverse grade school math word problems. We select from the error cases made by ChatGPT on the original dataset.
    \item \textbf{SciREX}, link: \url{https://github.com/allenai/SciREX}. SciREX is a challenging dataset for document-level information extraction based on a collection of full-length machine learning scientific papers. We formulate the original information extraction task into natural language question answering. 
    \item \textcolor{red}{\textbf{TemporalWiki/Wiki}.} It is difficult to dump only most recent (2022-) wikipedia knowledge. The on-going process is to dump the wikipedia (2023-04-20) and wikipedia (2022-04-20) and filter the changes out. It means we need to double the downloaded database and the filtering process is extremely time-consuming. An alternative way is to use our original way to generate some questions that ChatGPT itself cannot answer correctly with.
\end{itemize}

\subsubsection{Additional Data Sources}
\begin{itemize}
    \item \textcolor{red}{\textbf{WikiText}}. Use our generation template in version 1 to generate some detailed questions that ChatGPT itself cannot answer without some supportive materials. The biggest drawback is that we cannot get to know whether the answers are correct or not.
\end{itemize}
\subsubsection{Easy Questions}

\begin{itemize}
    \item \textbf{Math:} GSM8K;
    \item \textbf{SQL:} Flight, Coffee, Yelp, Airbnb;
    \item \textbf{Text Retriever:} SciREX~\cite{jain-etal-2020-scirex}, TemporalWiki;
    \item \textbf{Graph Toolkits:} DBLP.
\end{itemize}

\subsubsection{Hard Questions}
\ycz{From tool level, most questions are two-hop tool use, like SQL+Math, Retrieve+Math, Graph+Math}


% \subsection{Baselines}

% \subsubsection{Overall Performances}
% \begin{itemize}
%     \item \textbf{GPT-3.5-naive}. Test the ChatGPT performance without supportive materials. We expect the performance to be close to 0.
%     \item \textbf{GPT-3.5-COT}~\cite{neurips2022-cot}. Test the ChatGPT performance with chain-of-thoughts logic decomposition.
%     \item \textbf{Zero-shot ReAct} or \textbf{Few-shot ReAct}~\cite{yao2023react}. We will define the tools' usage and add the descriptions in the ReAct prompts or we just give some examples in the prompts.
%     \item \textbf{ToolFormer Prompting}~\cite{schick2023toolformer}. Follow the prompting style of ToolFormer to test the performances.
%     \item \textbf{Chamaleon}~\cite{lu2023chameleon} (optional?). 
%     \item \textbf{BMTools}~\cite{arxiv2023-toolsurvey}
% \end{itemize}

% \subsubsection{Tool Expert Performance}
% \begin{itemize}
    % \item \textbf{PAL}~\cite{gao2022pal} (math)
%     \item \textbf{Graph-ToolFormer}~\cite{zhang2023graphtoolformer} (graph)
%     \item \textbf{Replug}~\cite{shi2023replug} (text retriever)
%     \item \textbf{Self-Debugging}~\cite{chen2023teaching} (Text-to-SQL)
%     \item \textbf{Program-of-thoughts}~\cite{chen2022program} (use code thinking in tableQA - TATQA)
% \end{itemize}

% \subsection{Related Works}

% \begin{itemize}
%     \item \textbf{Methods:} \textcolor{red}{GeneGPT}~\cite{jin2023genegpt}, Visual ChatGPT~\cite{wu2023visual}, HuggingGPT~\cite{shen2023hugginggpt}
%     \item \textbf{Surveys:} Tool-using in foundation models~\cite{arxiv2023-toolsurvey}, augmented LLMs~\cite{arxiv2023-augmentedLLMsurvey};
%     \item \textbf{Benchmarks:} \textcolor{red}{API-Bank}~\cite{li2023apibank}
%     \item \textbf{Tools:} ChatGPT Plugins, AutoGPT, BabyAGI, etc.
% \end{itemize}
